Unplug and Play Language Models: Decomposing Experts in Language Models at Inference Time

Enabled by large-scale text corpora with huge parameters, pre-trained language models operate as multi-task experts using a single model architecture. However, recent studies have revealed that certain neurons play disproportionately important roles in solving specific tasks, suggesting that task-relevant substructures can be isolated and selectively activated for each task. Therefore, we introduce Decomposition of Experts (DoE), a novel framework that dynamically identifies and activates task-specific experts within a language model to reduce inference cost without sacrificing accuracy. We first define a task expert as a set of parameters that significantly influence the performance of a specific task and propose a four-step unplug-and-play process: (1) receiving a user request, (2) identifying the corresponding task expert, (3) performing inference using the expert-localized model, and (4) restoring the original model and waiting for the next task. Using attribution methods and prompt tuning, DoE isolates task-relevant neurons, minimizing computational overhead while maintaining task performance. We assume a setting where a language model receives user requests from five widely used natural language understanding benchmarks, processing one task at a time. In this setup, we demonstrate that DoE achieves up to a x1.73 inference speed-up with a 65% pruning rate, without compromising accuracy. Comparisons with various task expert localization methods reveal that DoE effectively identifies task experts, while ablation studies validate the importance of its components. Additionally, we analyze the effects of batch size, token count, and layer types on inference speed-up, providing practical insights for adopting DoE. The proposed framework is both practical and scalable, applicable to any transformer-based architecture, offering a robust solution for efficient task-specific inference.

==> fig_texts/algorithm1.tex <==
\algrenewcommand\algorithmicindent{1.5em}%
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\begin{algorithm}[t]
 \caption{\ours~Framework}\label{alg:cap}
\begin{algorithmic}[1]
\small 
\Require a dataset $\mathcal{D}_{\tau}$; a model $\mathcal{P}$; a prompt $p$
\Ensure a skill-localized model $\mathcal{P}_{\theta}$
\State $\mathcal{S} \gets$ false  \Comment{\scriptsize{Whether pruning is complete or not}}
\small
\For {epoch = $1,2,...,N$}
    \small
    \State $\mathcal{B} \gets $ split $\mathcal{D}_{train}$ into mini-batches of size $\beta$
    \For{each batch $b \in \mathcal{B}$}
        \State compute a batch loss $\mathcal{L}$
        \State $\theta_{P_{\tau}} \gets \theta_{P_{\tau}} - \lambda \triangledown_{\theta_{P_{\tau}}} \mathcal{L}$   \Comment{\scriptsize{prompt tuning}\small}
    \EndFor
    \If{$\mathcal{L}$ is converged}
        \State \textbf{break}
    \EndIf
\EndFor

\State $l \gets 0$
\State $r \gets 20$

\While {$l \leq r$}
\For {epoch = $1,2,...,N$}
    \If{$\mathcal{S}$ is false}
        \small
        \State $\mathcal{S} \gets$ true
        % \State sample a small subset $\Tilde{\mathcal{D}}_{train}$ and $\Tilde{\mathcal{D}}_{eval}$
        \For{each layer $l$ in $\mathcal{P}$}
            \State compute skill relevance $A_{i}(h^{l})$
        \EndFor
    \Else
        \State sort neuron indices by $A_{i}(h^{l})$
        \State get task-irrelevant neuron set $\mathcal{M}$ by $p$
        \State get $\Tilde{\mathcal{P}}$ by pruning $\mathcal{M}$ from $\mathcal{P}$
    \EndIf
\EndFor
\EndWhile
\Return $\mathcal{P}$

\end{algorithmic}
\label{algorithm:1}
\vspace{-0.02cm}
\end{algorithm}


==> fig_texts/algorithm_prev.tex <==
\algrenewcommand\algorithmicindent{1.5em}%
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\begin{algorithm}[H]
 \caption{\ours~Framework}
\begin{algorithmic}[1]
\small 
\Require a dataset $\mathcal{D}_{\tau}$; a model $\mathcal{P}$; a prompt $p$
\Ensure a skill-localized model $\mathcal{P}_{\theta}$
\State $\mathcal{S} \gets$ false  \Comment{\scriptsize{Whether pruning is complete or not}}
\small
\For {epoch = $1,2,...,N$}
    \small
    \State $\mathcal{B} \gets $ split $\mathcal{D}_{train}$ into mini-batches of size $\beta$
    \For{each batch $b \in \mathcal{B}$}
        \State compute a batch loss $\mathcal{L}_{\mathcal{P}}(b)$
        \State $\theta_{P} \gets \theta_{P} - \lambda \triangledown_{\theta} \mathcal{L}_{\mathcal{P}}(b)$   \Comment{\scriptsize{prompt tuning}\small}
    \EndFor
    \If{$\mathcal{L}_{\mathcal{P}}$ is converged}
        \If{$\mathcal{S}$ is false}
            \small
            \State $\mathcal{S} \gets$ true
            % \State sample a small subset $\Tilde{\mathcal{D}}_{train}$ and $\Tilde{\mathcal{D}}_{eval}$
            \For{each layer $l$ in $\mathcal{P}$}
                \State compute skill relevance $A_{i}(h^{l})$
            \EndFor
        \Else
            \State sort neuron indices by $A_{i}(h^{l})$
            \State get task-irrelevant neuron set $\mathcal{M}$ by $p$
            \State get $\Tilde{\mathcal{P}}$ by pruning $\mathcal{M}$ from $\mathcal{P}$
        \EndIf
    \EndIf
\EndFor
\Return $\mathcal{P}$

\end{algorithmic}
\label{algorithm:1}
\vspace{-0.02cm}
\end{algorithm}


==> fig_texts/attribution_num.tex <==
\begin{figure}[H]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=7.0cm]{fig_files/attribution_num.pdf}}
%  \vspace{1.5cm}
\end{minipage}
\caption{\textbf{Experimental results for varying numbers of data samples to quantify skill relevance.} We plot the mean accuracy (± one standard deviation for three trials) of BERT for IMDB and MRPC datasets.}
\label{fig:attribution_num}
%
\end{figure}
% \vspace{-5mm}

==> fig_texts/fig_margin.tex <==
\begin{figure}[H]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=7.0cm]{fig_files/margin.pdf}}
%  \vspace{1.5cm}
\end{minipage}
\caption{\textbf{Hyper-parameter experiments for the margin ($\psi$).} The red-dotted line is the baseline performance (Prefix-tuning). The size of each circle represents the inference speed, and the percentage annotated in each circle indicates the pruning rate.}
\label{fig:margin}
\end{figure}

==> fig_texts/fig_modelsize.tex <==
\begin{figure}[H]
\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=\columnwidth]{fig_files/model_size.pdf}}
%  \vspace{1.5cm}
\end{minipage}
\caption{\textbf{Temperature search results for Local Confusion and Global Confusion.} X-axis corresponds to temperature and Y-axis corresponds to the difference in golden logit reduction between IG and DiscGrad.}
\label{fig:fig2}
%
\end{figure}
% \vspace{-5mm}

==> fig_texts/table2.tex <==
\begin{table}[h]
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{ccccccc}
% \begin{tabular}{c{1cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}} 
\toprule
 Model &  Method & SST-2 &  IMDB &  AGNews &  MRPC &  CB \\ \midrule
\multirow{2}{*}{\makecell{BERT}} & \textbf{Pruning rates} & 36.7\% \small & 38.3\% \small & 55.0\% \small & 65.0\% \small & 65.0\% \small  \\
& \textbf{Speed-up} & \color{myred}$\times 1.29$ & \color{red}$\times 1.30$ & \color{red}$\times 1.43$ & \color{red}$\times 1.73$ & \color{red}$\times 1.72$  \\
\bottomrule 



\multirow{2}{*}{\makecell{RoBERTa}} & \textbf{Pruning rates} & 30.0\% \small & 36.7\% \small & 61.7\% \small & 58.3\% \small & 63.3\% \small  \\
& \textbf{Speed-up} & \color{myred}$\times 1.18$ & \color{myred}$\times 1.23$ & \color{myred}$\times 1.25$ & \color{red}$\times 1.39$ & \color{red}$\times 1.53$ \\
\bottomrule 

\end{tabular}
}
\vspace{-0.1cm}
\caption{
\textbf{Task Neuron Localized Prompt Tuning Results.} \textit{Pruning Rate (\%)} and \textit{Speed up ($\times$)} mean the ratio of neurons deactivated after applying our method and the inference speed up compared to the Prompt-tuning, respectively.
The values in parenthesis are the number of pruned parameters.
The pruning rates are calculated based on the maximum number of prunable parameters.
}
% \vspace{-0.5cm}
\label{table2}
\end{table}


==> texts/limitations.tex <==
Our framework accelerates the inference speed of language models, identifying the optimal subnetwork for utilizing language models.
However, while our approach exhibited comparable performance and occasionally slightly superior results to the existing prompt tuning method, these improvements were not consistent across overall task performance.
In addition, our experiments are limited to five widely-used natural language understanding datasets; thus, we should extend to a wide range of datasets to validate the applicability of our framework.
Furthermore, we select feed-forward networks to localize task neurons in language models since they are adequate for inference speed acceleration.
However, the entire modules in Transformer should be considered as a localization target to achieve the extreme inference speed up; we leave this point as future research.
